Observations of CH$_3$OH and CH$_3$CHO in a Sample of Protostellar Outflow Sources

Iram 30-m Observations towards eight protostellar outflow sources were taken in the 96-\SI{176}{\giga\hertz} range. Transitions of CH$_3$OH and CH$_3$CHO were detected in seven of them. The integrated emission of the transitions of each species that fell into the observed frequency range were measured and fit using RADEX and LTE models. Column densities and gas properties inferred from this fitting are presented. The ratio of the A and E-type isomers of CH$_3$OH indicate that the methanol observed in these outflows was formed on the grain surface. Both species demonstrate a reduction of terminal velocity in their line profiles in faster outflows, indicating destruction in the post-shock gas phase. This destruction, and a near constant ratio of the CH$_3$OH and CH$_3$CHO column densities imply it is most likely that CH$_3$CHO also forms on the grain surface.

==> spectraplots.tex <==
\figsetstart
\figsetnum{1}
\figsettitle{Plots of all detected lines of CH$_3$OH and CH$_3$CHO in each source.}
\figsetgrpstart
\figsetgrpnum{1}
\figsetgrptitle{Detected transitions of CH$_3$OH in IRAS2A-B}
\figsetplot{figures/stamps/stamp-iras2a-b-ch3oh1.pdf}
\figsetgrpnote{Detected transitions of CH$_3$OH in IRAS2A-B. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{2}
\figsetgrptitle{Detected transitions of CH$_3$CHO in IRAS2A-R}
\figsetplot{figures/stamps/stamp-iras2a-r-ch3cho1.pdf}
\figsetgrpnote{Detected transitions of CH$_3$CHO in IRAS2A-R. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{3}
\figsetgrptitle{Detected transitions of CH$_3$CHO in IRAS2A-R}
\figsetplot{figures/stamps/stamp-iras2a-r-ch3cho2.pdf}
\figsetgrpnote{Detected transitions of CH$_3$CHO in IRAS2A-R. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{4}
\figsetgrptitle{Detected transitions of CH$_3$CHO in IRAS2A-R}
\figsetplot{figures/stamps/stamp-iras2a-r-ch3cho3.pdf}
\figsetgrpnote{Detected transitions of CH$_3$CHO in IRAS2A-R. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{5}
\figsetgrptitle{Detected transitions of CH$_3$OH in IRAS2A-R}
\figsetplot{figures/stamps/stamp-iras2a-r-ch3oh1.pdf}
\figsetgrpnote{Detected transitions of CH$_3$OH in IRAS2A-R. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{6}
\figsetgrptitle{Detected transitions of CH$_3$OH in IRAS2A-R}
\figsetplot{figures/stamps/stamp-iras2a-r-ch3oh2.pdf}
\figsetgrpnote{Detected transitions of CH$_3$OH in IRAS2A-R. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{7}
\figsetgrptitle{Detected transitions of CH$_3$OH in IRAS2A-R}
\figsetplot{figures/stamps/stamp-iras2a-r-ch3oh3.pdf}
\figsetgrpnote{Detected transitions of CH$_3$OH in IRAS2A-R. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{8}
\figsetgrptitle{Detected transitions of CH$_3$OH in IRAS2A-R}
\figsetplot{figures/stamps/stamp-iras2a-r-ch3oh4.pdf}
\figsetgrpnote{Detected transitions of CH$_3$OH in IRAS2A-R. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{9}
\figsetgrptitle{Detected transitions of CH$_3$CHO in IRAS4A-B}
\figsetplot{figures/stamps/stamp-iras4a-b-ch3cho1.pdf}
\figsetgrpnote{Detected transitions of CH$_3$CHO in IRAS4A-B. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{10}
\figsetgrptitle{Detected transitions of CH$_3$CHO in IRAS4A-B}
\figsetplot{figures/stamps/stamp-iras4a-b-ch3cho2.pdf}
\figsetgrpnote{Detected transitions of CH$_3$CHO in IRAS4A-B. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{11}
\figsetgrptitle{Detected transitions of CH$_3$OH in IRAS4A-B}
\figsetplot{figures/stamps/stamp-iras4a-b-ch3oh1.pdf}
\figsetgrpnote{Detected transitions of CH$_3$OH in IRAS4A-B. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{12}
\figsetgrptitle{Detected transitions of CH$_3$OH in IRAS4A-B}
\figsetplot{figures/stamps/stamp-iras4a-b-ch3oh2.pdf}
\figsetgrpnote{Detected transitions of CH$_3$OH in IRAS4A-B. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{13}
\figsetgrptitle{Detected transitions of CH$_3$OH in IRAS4A-B}
\figsetplot{figures/stamps/stamp-iras4a-b-ch3oh3.pdf}
\figsetgrpnote{Detected transitions of CH$_3$OH in IRAS4A-B. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{14}
\figsetgrptitle{Detected transitions of CH$_3$OH in IRAS4A-B}
\figsetplot{figures/stamps/stamp-iras4a-b-ch3oh4.pdf}
\figsetgrpnote{Detected transitions of CH$_3$OH in IRAS4A-B. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{15}
\figsetgrptitle{Detected transitions of CH$_3$CHO in IRAS4A-R}
\figsetplot{figures/stamps/stamp-iras4a-r-ch3cho1.pdf}
\figsetgrpnote{Detected transitions of CH$_3$CHO in IRAS4A-R. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{16}
\figsetgrptitle{Detected transitions of CH$_3$OH in IRAS4A-R}
\figsetplot{figures/stamps/stamp-iras4a-r-ch3oh1.pdf}
\figsetgrpnote{Detected transitions of CH$_3$OH in IRAS4A-R. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{17}
\figsetgrptitle{Detected transitions of CH$_3$OH in IRAS4A-R}
\figsetplot{figures/stamps/stamp-iras4a-r-ch3oh2.pdf}
\figsetgrpnote{Detected transitions of CH$_3$OH in IRAS4A-R. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{18}
\figsetgrptitle{Detected transitions of CH$_3$OH in IRAS4A-R}
\figsetplot{figures/stamps/stamp-iras4a-r-ch3oh3.pdf}
\figsetgrpnote{Detected transitions of CH$_3$OH in IRAS4A-R. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{19}
\figsetgrptitle{Detected transitions of CH$_3$CHO in L1157-B2}
\figsetplot{figures/stamps/stamp-l1157-b2-ch3cho1.pdf}
\figsetgrpnote{Detected transitions of CH$_3$CHO in L1157-B2. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{20}
\figsetgrptitle{Detected transitions of CH$_3$CHO in L1157-B2}
\figsetplot{figures/stamps/stamp-l1157-b2-ch3cho2.pdf}
\figsetgrpnote{Detected transitions of CH$_3$CHO in L1157-B2. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{21}
\figsetgrptitle{Detected transitions of CH$_3$OH in L1157-B2}
\figsetplot{figures/stamps/stamp-l1157-b2-ch3oh1.pdf}
\figsetgrpnote{Detected transitions of CH$_3$OH in L1157-B2. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{22}
\figsetgrptitle{Detected transitions of CH$_3$OH in L1157-B2}
\figsetplot{figures/stamps/stamp-l1157-b2-ch3oh2.pdf}
\figsetgrpnote{Detected transitions of CH$_3$OH in L1157-B2. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{23}
\figsetgrptitle{Detected transitions of CH$_3$OH in L1157-B2}
\figsetplot{figures/stamps/stamp-l1157-b2-ch3oh3.pdf}
\figsetgrpnote{Detected transitions of CH$_3$OH in L1157-B2. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{24}
\figsetgrptitle{Detected transitions of CH$_3$OH in L1157-B2}
\figsetplot{figures/stamps/stamp-l1157-b2-ch3oh4.pdf}
\figsetgrpnote{Detected transitions of CH$_3$OH in L1157-B2. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{25}
\figsetgrptitle{Detected transitions of CH$_3$OH in L1157-R}
\figsetplot{figures/stamps/stamp-l1157-r-ch3oh1.pdf}
\figsetgrpnote{Detected transitions of CH$_3$OH in L1157-R. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{26}
\figsetgrptitle{Detected transitions of CH$_3$OH in L1448-B2}
\figsetplot{figures/stamps/stamp-l1448-b2-ch3oh1.pdf}
\figsetgrpnote{Detected transitions of CH$_3$OH in L1448-B2. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\figsetgrpend
\figsetend
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figures/stamps/stamp-iras2a-b-ch3oh1.pdf}
\caption{Detected transitions of CH$_3$OH in IRAS2A-B. The grey shaded range is the velocity interval over which the emission was integrated. The dashed horizontal lines show the rms noise level and three times that value. The vertical line shows the position of the peak.}
\label{fig:stamps}
\end{figure*}
